How to Verify Any (Reasonable) Distribution Property: Computationally Sound Argument Systems for Distributions

As statistical analyses become more central to science, industry and society, there is a growing need to ensure correctness of their results. Approximate correctness can be verified by replicating the entire analysis, but can we verify without replication? Building on a recent line of work, we study proof-systems that allow a probabilistic verifier to ascertain that the results of an analysis are approximately correct, while drawing fewer samples and using less computational resources than would be needed to replicate the analysis. We focus on distribution testing problems: verifying that an unknown distribution is close to having a claimed property. Our main contribution is a interactive protocol between a verifier and an untrusted prover, which can be used to verify any distribution property that can be decided in polynomial time given a full and explicit description of the distribution. If the distribution is at statistical distance $\varepsilon$ from having the property, then the verifier rejects with high probability. This soundness property holds against any polynomial-time strategy that a cheating prover might follow, assuming the existence of collision-resistant hash functions (a standard assumption in cryptography). For distributions over a domain of size $N$, the protocol consists of $4$ messages and the communication complexity and verifier runtime are roughly $\widetilde{O}\left(\sqrt{N} / \varepsilon^2 \right)$. The verifier's sample complexity is $\widetilde{O}\left(\sqrt{N} / \varepsilon^2 \right)$, and this is optimal up to $\polylog(N)$ factors (for any protocol, regardless of its communication complexity). Even for simple properties, approximately deciding whether an unknown distribution has the property can require quasi-linear sample complexity and running time. For any such property, our protocol provides a quadratic speedup over replicating the analysis.

==> fig-label-inv-protocol.tex <==
\renewcommand{\figurename}{Protocol}
\captionsetup{labelfont=bf}
\begin{figure}[!h]
  \thisfloatpagestyle{empty}
  \begin{boxedminipage}{\textwidth}
    \small \medskip \noindent
\caption{\bf Verifying Label-Invariant Distribution Properties} \label{fig:label-inv-prot}
\medskip
    \textbf{Input:} label-invariant distribution property $\left(\mathcal{P}\right)$ that admits an approximate decision procedure (see Definition ??), domain size parameter $N\in\mathbb{N}$, security parameter $\kappa\in\mathbb{N}$, distance parameters $\delta_c,\delta_f\in(0,1)$, such that $\delta_f-\delta_c=\rho>\frac{1}{\poly(N)}$, and black-box sample access to a distribution $D$ over domain $[N]$.  \\
    \textbf{Goal: } accept w.h.p. if $\SD(D,\mathcal{P}_N)\leq \delta_c$; reject w.h.p. if $\SD(D,\mathcal{P}_N)\geq \delta_f$.

    %\textbf{Goal:} output .\\

    \begin{enumerate}
        \item V-P: run Protocol \ref{fig:full-prot}, reject if the protocol resulted in rejection.
        \item V: run ?? to draw $\poly\left(log(N),\rho\right)$ samples from $Q$, and obtain $Q[x]$ for every $x$ sampled. Compute the $\rho/3$-approximate probability histogram of $Q$ based on the sample as explain in 
    \end{enumerate}
 
    \smallskip
  \end{boxedminipage}
\end{figure}


==> fig-reconstruction-circuit.tex <==
\renewcommand{\figurename}{Algorithm}
\captionsetup{labelfont=bf}
\begin{figure}[!h]
  \thisfloatpagestyle{empty}
  \begin{boxedminipage}{\textwidth}
    \small \medskip \noindent
\caption{\bf Distribution Reconstruction Algorithm} \label{fig:recon-alg}
\medskip
    \textbf{Input:} string $X\in\left\{0,1\right\}^M$, parameter $\gamma\in(0,1)$, as well as hash function $h,h_\gamma$.\\
    \textbf{Output:} if didn't reject, outputs $(D^X_x)_{x\in [N]}$. 
    \begin{enumerate}
        \item For every $x\in[N]$, compute $t_x=\max\left\{t:X\left(h(x,t)\right)=1\right\}$, by querying $X$ in locations $h(x,1), h(x,2),\dots$, until reaching $t$ such that $X\left(h(x,t)\right)=0$ or $t=\left\lceil N^{1-f}/\gamma\right\rceil$, then set $t_x=t-1$, and $D^X_x=\frac{\gamma}{N}\cdot t_x -\frac{\gamma_x}{N}$. For every $y\in[M]$ keep a counter $c_y$ that counts how many pairs $(x,t)$ satisfy $h(x,t)=y$ and $t\leq t_x$. If there exists $c_y$ such that $c_y\geq \log N$, reject.
        \item For every $x\in[N]$, check that the set of locations $\left\{h(x,t):t\in\left\{t_x+1,t_x+2,\dots,N^{1-f}/\gamma\right\}\right\}$ does not contain $\log N$ consecutive $1$'s: i.e. for every $i_0\in \left\{t_x+1,\dots,N^{1-f}/\gamma-\log N\right\}$ and $V_{t_x+i_0}=\left\{(x,t_x+i):i\in\left\{1,2,\dots \log N\right\}\right\}$, check that there exists $(x',t')\in V_{t_x+i_0}$ such that $y=h(x',t')$ and $X(y)=0$. Reject otherwise.
        \item Output $\left(D^X_x\right)_{x\in[N]}$
    \end{enumerate}
 
    \smallskip
  \end{boxedminipage}
\end{figure}


==> label-inv-protocol.tex <==
\renewcommand{\figurename}{Protocol}
\captionsetup{labelfont=bf}
\begin{figure}[!h]
  \thisfloatpagestyle{empty}
  \begin{boxedminipage}{\textwidth}
    \small \medskip \noindent
\caption{\bf Verifying Label-Invariant Distribution Properties} \label{fig:label-inv-prot}
\medskip
    \textbf{Input:} label-invariant distribution property $\left(\mathcal{P}\right)$ that admits an approximate decision procedure (see Definition ??), domain size parameter $N\in\mathbb{N}$, security parameter $\kappa\in\mathbb{N}$, distance parameters $\delta_c,\delta_f\in(0,1)$, such that $\delta_f-\delta_c=\rho>\frac{1}{\poly(N)}$, and black-box sample access to a distribution $D$ over domain $[N]$.  \\
    \textbf{Goal: } accept w.h.p. if $\SD(D,\mathcal{P}_N)\leq \delta_c$; reject w.h.p. if $\SD(D,\mathcal{P}_N)\geq \delta_f$.

    %\textbf{Goal:} output .\\

    \begin{enumerate}
        \item V-P: run Protocol \ref{fig:full-prot}, reject if the protocol resulted in rejection.
        \item V: run ?? to draw $\poly\left(log(N),\rho\right)$ samples from $Q$, and obtain $Q[x]$ for every $x$ sampled. Compute the $\rho/3$-approximate probability histogram of $Q$ based on the sample as explain in 
    \end{enumerate}
 
    \smallskip
  \end{boxedminipage}
\end{figure}

